Towards Chip-on-Chip Neuroscience: Fast Mining of Frequent Episodes Using Graphics Processors

Computational neuroscience is being revolutionized with the advent of multi-electrode arrays that provide real-time, dynamic, perspectives into brain function. Mining event streams from these chips is critical to understanding the firing patterns of neurons and to gaining insight into the underlying cellular activity. We present a GPGPU solution to mining spike trains. We focus on mining frequent episodes which captures coordinated events across time even in the presence of intervening background/"junk" events. Our algorithmic contributions are two-fold: MapConcatenate, a new computation-to-core mapping scheme, and a two-pass elimination approach to quickly find supported episodes from a large number of candidates. Together, they help realize a real-time "chip-on-chip" solution to neuroscience data mining, where one chip (the multi-electrode array) supplies the spike train data and another (the GPGPU) mines it at a scale unachievable previously. Evaluation on both synthetic and real datasets demonstrate the potential of our approach.

==> tex/repeatability.tex <==
\section{Repeatability}
We are committed to repeatability and have hosted all datasets and
implementations presented here at the public website:
http://neural-code.cs.vt.edu/gpgpu/. Supplementary information is also
provided at this site in support of the claims and conclusions of this
paper.
%\narenc{Give a URL to codes, algorithm implementations, and results.
%KDD strongly recommends this.} Promise that we will host it on a Google
%code page after the paper is accepted.


